GelTip Tactile Sensor for Dexterous Manipulation in Clutter

Tactile sensing is an essential capability for robots that carry out dexterous manipulation tasks. While cameras, Lidars and other remote sensors can assess a scene globally and instantly, tactile sensors can reduce their measurement uncertainties and gain information about the local physical interactions between the in-contact objects and the robot, that are often not accessible via remote sensing. Tactile sensors can be grouped into two main categories: electronic tactile skins and camera based optical tactile sensors. The former are slim and can be fitted to different body parts, whereas the latter assume a more prismatic shape and have much higher sensing resolutions, offering a good advantage for being used as robotic fingers or fingertips. One of such optical tactile sensors is our GelTip sensor that is shaped as a finger and can sense contacts on any location of its surface. As such, the GelTip sensor is able to detect contacts from all the directions, like a human finger. To capture these contacts, it uses a camera installed at its base to track the deformations of the opaque elastomer that covers its hollow, rigid and transparent body. Thanks to this design, a gripper equipped with GelTip sensors is capable of simultaneously monitoring contacts happening inside and outside its grasp closure. Experiments carried out using this sensor demonstrate how contacts can be localised, and more importantly, the advantages, and even possibly a necessity, of leveraging all-around touch sensing in dexterous manipulation tasks in clutter where contacts may happen at any location of the finger. All the materials for the fabrication of the GelTip sensor can be found at https://danfergo.github.io/geltip/

==> aboutauthors.tex <==
\begin{frontmatter}
\chapter*{Biography}
\end{frontmatter}

\begin{biography}

  \section*{Sir Stanley Davidson (1894--1981)}

  One or more blank lines denote the end of a paragraph.  The ends of\index{index}
  words and sentences are marked by spaces. It doesn't matter how many
  spaces you type; one is as good as 100.  The end of a line counts as
  a space.

\end{biography}


==> chapter2.tex <==
\cleardoublepage

\begin{frontmatter}
\chapter{Chapter Title\footnote{This is chapter footnote}}\label{chap2}
\subchapter{Chapter Subtitle}

\begin{aug}
\author[addressrefs={ad1,ad2}]%
  {\fnm{Firstname}   \snm{Surname}}%
  %{\fnm{Firstname}   \snm{Surname}\footnote{This is author footnote}}%
\author[addressrefs={ad2}]%
 {\fnm{Firstname} \snm{Surname}}%
\address[id=ad1]%
  {Short Address}%
\address[id=ad2]%
  {Long Address}%
\end{aug}


% \minitoc

%
\begin{chapterpoints}%[Chapter Points]
\item The ends of words and sentences are marked by spaces. It doesn't
  matter how many spaces you type; one is as good as 100.  The end of
  a line counts as a space.

\item The ends of words and sentences are marked by spaces. It doesn't
  matter how many spaces you type; one is as good as 100.  The end of
  a line counts as a space.
\end{chapterpoints}

\begin{dispquote}

  The ends of words and sentences are marked by spaces. It doesn't
  matter how many spaces you type; one is as good as 100.  The end of
  a line counts as a space.

  The ends of words and sentences are marked by spaces. It doesn't
  matter how many spaces you type; one is as good as 100.  The end of
  a line counts as a space.
  
  \source{Name}

\end{dispquote}

\end{frontmatter}


\section{Section title}\label{sec2.1}


==> contributors.tex <==
%% Contributors list %%
\begin{frontmatter}
\chapter*{Contributors}
\end{frontmatter}

\begin{contributorslist}
  \name{Greg N. Gregoriou} is Professor of Finance in the School of
  Business and Economics at State University of New York at
  Plattsburgh. He obtained his Ph.D. (finance) from the University of
  Quebec at Montreal and is hedge-fund editor for the peer-reviewed
  scientific journal Derivatives Use, Trading and Regulation and
  editorial board member for the Journal of Wealth Management, and the
  Journal of Risk and Financial Institutions. He has written more than
  50 articles on hedge funds and managed futures in various U.S. and
  U.K. peer-reviewed publications, including (among others) the
  Journal of Portfolio Management, Journal of Derivatives Accounting,
  Journal of Futures Markets, European Journal of Operational
  Research, Annals of Operations Research, European Journal of
  Finance, and Journal of Asset Management. He has edited 18 books for
  Elsevier, Wiley, Palgrave-MacMillan, and Risk and has coauthored one
  book for Wiley.

  \name{Donald F. Dansereau} Department of Psychology, Texas Christian
  University, Fort worth, Texas

  \name{Ruth Garner} Department of Educational Psychology, Texas A \&
  M University, College Station, Texas
\end{contributorslist}



==> dedication.tex <==
  %% Dedication page
\begin{dedication}
  %% Dedication
  %% can be few\\
  %% lines long
\end{dedication}


==> listoffigures.tex <==
\begin{frontmatter}
\chapter*{List of Figures}
\end{frontmatter}

\listoffigures


==> part.tex <==
\cleardoublepage
\begin{frontmatter}
%\part{}
\end{frontmatter}

% Text ...


==> part1.tex <==
\begin{frontmatter}
\part{Part title}\label{part1}
\end{frontmatter}




==> preface.tex <==
\cleardoublepage
\begin{frontmatter}
\chapter*{Preface}%
%\addcontentsline{toc}{schapter}{Preface}
\end{frontmatter}


 The ends of words and sentences are marked by spaces. It doesn't
 matter how many spaces you type; one is as good as 100.  The end of
 a line counts as a space.

 The ends of words and sentences are marked by spaces. It doesn't
 matter how many spaces you type; one is as good as 100.  The end of
 a line counts as a space.

 The ends of words and sentences are marked by spaces. It doesn't
 matter how many spaces you type; one is as good as 100.  The end of
 a line counts as a space.

\source%
{%
  \author{Name}\\%
  % \address{Location}\\%
  % \date{Month Year}%
}


==> references.tex <==
%\begin{frontmatter}
%  \chapter*{References}
%  \markboth{References}{References}
%\end{frontmatter}


\bibliographystyle{elsarticle-harv} 
\bibliography{references}

%\begin{thebibliography}{10}

% \bibitem{..}
% \bibitem[]{..}

% \end{thebibliography}

==> tableofcontents.tex <==
%% Table of Contents %%
\begin{frontmatter}
\chapter*{Contents}
\end{frontmatter}

\tableofcontents


==> titlepage.tex <==
%% Title Page %%
\begin{titlepage}%
  \begin{titlepagerule}
    \title{Book title}
    %\subtitle{Book Subtitle}
    %\volume{2}
  \end{titlepagerule}

  \edition{2nd edition}

%  \editedby{Edited by}

  \author{Author Firstname  Surname}
  \address{Author Address\\Department of Chemistry\\University of Florida}

  \author{Author Firstname  Surname}
  \address{Author Address}
\end{titlepage}

